HashPoint: Accelerated Point Searching and Sampling for Neural Rendering

In this paper, we address the problem of efficient point searching and sampling for volume neural rendering. Within this realm, two typical approaches are employed: rasterization and ray tracing. The rasterization-based methods enable real-time rendering at the cost of increased memory and lower fidelity. In contrast, the ray-tracing-based methods yield superior quality but demand longer rendering time. We solve this problem by our HashPoint method combining these two strategies, leveraging rasterization for efficient point searching and sampling, and ray marching for rendering. Our method optimizes point searching by rasterizing points within the camera's view, organizing them in a hash table, and facilitating rapid searches. Notably, we accelerate the rendering process by adaptive sampling on the primary surface encountered by the ray. Our approach yields substantial speed-up for a range of state-of-the-art ray-tracing-based methods, maintaining equivalent or superior accuracy across synthetic and real test datasets. The code will be available at https://jiahao-ma.github.io/hashpoint/.

==> sec/4_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\noindent \textbf{Ours \textit{vs.} traditional point cloud searching.} Retrieving the neighboring point cloud to a camera ray is non-trivial. A straightforward method is to compare all rays with all points, leading to high computation costs. Common approaches employ space partitioning to expedite the search. Below, taking an example with $n$ points and $m$ rays with an average of $q$ points falling in the radius $\delta$ of each ray, we introduce the search processes and the corresponding complexity of these algorithms. 

\begin{figure}[ht]
\centering
\includegraphics[width=1.0\linewidth]{figures/sampling.jpg}
\caption{Point cloud selection strategies. \textbf{A}: \textit{K-NP Extract}: extracting \textit{K} nearest point features per ray. \textbf{B}:\textit{Depth Map Sampling} : sampling based on dense depth maps. \textbf{C}: \textit{Multi-Surface Sampling} : uniform sampling over multiple surfaces. \textbf{D}: \textit{Our method}: sampling on the primary surface. }
\label{fig:sampling}
\end{figure}

\begin{itemize}

    \item \textbf{KD-Tree} \cite{original_kdtree}: a space-partitioning data structure for organizing points in a k-dimensional space. To locate points near a ray using this structure, two common strategies exist: (1) Sample uniformly along the ray followed by radius searches at each sample point, and (2) leverage sub-tree bounding boxes in the KD-Tree and apply axis-aligned bounding box (AABB \cite{geometric_tools}) for intersections, then compare points in intersecting sub-trees. Building the KD-Tree needs to iterate $n$ points with the complexity of $\mathcal{O}(n)$, and in the case of searching points for $m$ rays, the complexity of finding all intersecting sub-trees and retrieving $q$ points within the cylinder of rays is $\mathcal{O}(mlog(n) + mq)$.

    \item \textbf{Octree} \cite{Octree}: a tree data structure used to partition a three-dimensional space by recursively subdividing it into eight octants. This strategy for finding points near a ray is similar to the KD-Tree mentioned above, and the complexity is the same - constructing an Octree requires $\mathcal{O}(n)$, while searching requires $\mathcal{O}(mlog(n) + mq)$.
    
    \item \textbf{Uniform grid} \cite{introduction_ray_tracing}: a data structure that divides space into regular grids and allocates data to each grid cell. Building this data structure requires traversing all points with complexity $\mathcal{O}(n)$. For searches, using algorithms like 3DDA \cite{voxel_traversal} or AABB to find intersecting voxel with rays, the complexity is $\mathcal{O}(mg + mq)$, where $g$ is the number of grid cells per dimension.

    \item \textbf{Ours}: In the light of design, the previous method has the ray actively seeking point cloud in 3D space. In contrast, our method lets point cloud seek rays. To facilitate rapid query, an acceleration structure in the form of a hashtable is constructed by iterating all points followed by searching via hashtable looking up. The complexity of this process is $\mathcal{O}(n + mq)$.
\end{itemize}

\noindent \textbf{Ours \textit{vs.} existing point cloud selection strategies.} The selection of point cloud, such as the number and location, directly determines and quality and efficiency of rendering. As shown in Fig. \ref{fig:sampling}, we compare various methods of point cloud selection as follows:
\begin{itemize}
    \item ``\textit{K-NP Extract}'' \cite{papr, pointersect, nplf} refers to extracting the nearest \textit{K} point features around a ray to predict its color. Due to the density of the point cloud, the \textit{K} nearest points often don't necessarily fall on the primary surface, leading to feature noise. 
    \item ``\textit{Depth Map Sampling}'' \cite{diner, pointslam} refers to using sensor depth or MVS to predict the depth of neighboring views to assist sampling. Although this method is highly efficient, it relies on dense depth maps and also faces the issue of redundant sampling on multiple surfaces (especially in the case of relying on nearby views with depth input). 
    \item ``\textit{Multi-Surface Sampling}'' \cite{pointnerf} involves finding all surfaces intersecting with the ray and then uniformly sampling on them. The method provides the best result at the cost of extensive computation. 
    \item \textit{Our method} serves as a trade-off, balancing the precision and efficiency by sampling on the primary surface. 
\end{itemize}








